A Tale of Two Models: Constructing Evasive Attacks on Edge Models

Full-precision deep learning models are typically too large or costly to deploy on edge devices. To accommodate to the limited hardware resources, models are adapted to the edge using various edge-adaptation techniques, such as quantization and pruning. While such techniques may have a negligible impact on top-line accuracy, the adapted models exhibit subtle differences in output compared to the original model from which they are derived. In this paper, we introduce a new evasive attack, DIVA, that exploits these differences in edge adaptation, by adding adversarial noise to input data that maximizes the output difference between the original and adapted model. Such an attack is particularly dangerous, because the malicious input will trick the adapted model running on the edge, but will be virtually undetectable by the original model, which typically serves as the authoritative model version, used for validation, debugging and retraining. We compare DIVA to a state-of-the-art attack, PGD, and show that DIVA is only 1.7-3.6% worse on attacking the adapted model but 1.9-4.2 times more likely not to be detected by the the original model under a whitebox and semi-blackbox setting, compared to PGD.

==> defense.tex <==
\section{Possible \name Defenses} \label{sec:defenses}

\name is a particularly sticky type of attack in that, by design, the \q model always subtly deviates from the \fp model, and therefore \name can leverage differential testing to effectively locate the deviations. To understand how powerful \name is, we build or consider five defenses, including both existing robust training methods and a new method designed specifically for \name. These methods adopt the state-of-the-art techniques such as Minimax robust training~\cite{minmax_robust_training}, QAT~\cite{JacobKCZTHAK18}, and knowledge distillation~\cite{BaC14,PolinoPA18}. Unfortunately, as our evaluation (\S\ref{sec:eval-defense}) shows, none of these defenses is effective against \name because the deviations of the \fp and \q models always exist.

% We implemented three defensive methods with different combinations among Minimax robust training, QAT and knowledge distillation. Since \name is targeting the quatized model while keeping the \fp model unaware of the attack, our goal is to make the \q model more robust.

\paragraph{Minimax PGD robust training.}
This method applies robust training on the \fp model with the PGD attack before quantization. The primary reason to apply robustness to the \fp model, not \q model, is to make the two models more consistent. If we were to apply this method to the \q model only, it would differ even more from the \fp model.
% In addition, as explained in \S\ref{sec:quantization}, robust training almost always applies to the \fp model because it is expensive and requires the model to be differentiable.

Following Equation~\ref{eq:robust}, we arrive at the following a Minimax optimization problem

\begin{equation}\label{defense_method1}
    min_{\theta_f}\,max_{A \leq \epsilon}L_{f}(\theta_f, x + A, y)
\end{equation}

\noindent
where $\theta_f$ are the parameters and $L_f$ the loss function of the \fp model. The optimization goal is to adjust the \fp model's parameters $\theta_f$ to minimize the maximum damage that an attacker may inflict via any perturbation $A$ within the bound $\epsilon$.

Operationally, each training iteration uses PGD to maximize the loss based on the samples in the current mini-batch. After training converges, we apply quantization-aware training on the resultant \fp model to derive the \q model.

\paragraph{Minimax \name quantization aware training.}

This new method is fully aware of the \name attacks. It applies Minimax robust training to the \q model to reduce deviation while keeping the \fp model untouched. Since it requires the model to be differentiable and adjusts the parameters, we combine it with quantization-aware training.

Following Equation~\ref{eq:robust}, we arrive at the following Minimax optimization problem

\begin{equation}\label{defense_method2}
    min_{\theta_q}\,max_{A \leq \epsilon}L_{\name}(\theta_q, x + A, y)
\end{equation}

\noindent
where $\theta_q$ are the parameters of the \q model and $L_{\name}$ the loss function of the \name attack (\S\ref{sec:whitebox}). The idea is to adjust the parameters of the \q model to minimize the maximum difference that the \name attack may inflict on the predictions of the two models.

\paragraph{Distillation}

We apply distillation to make the \q model (student) behave more like the \fp model (teacher). Some prior work (Papernot \etal~\cite{distillation-defense}) shows this method may help improve the \q model's robustness against adversarial attacks that target the \q model alone. 
Our experiments show that distillation alone does not alter the effectiveness of \name because it aligns the two models only on clean images, agreeing with the results reported by Carlini \etal~\cite{carlini2016defensive} that defensive distillation is ineffective, at least for our use case. For conciseness, we omit reporting the defensive distillation results in \S\ref{sec:eval-defense}.

\paragraph{Minimax \name quantization aware training with distillation.}

This method combines the preceding two methods. Each training iteration first solves the Minimax \name problem and then generates \name adversarial samples for distillation. The idea is to use distillation to further align the \fp and \q models on the \name-generated adversarial samples. The number of \name adversarial samples generated varies from 20 to 50 depending on the model.

% we also apply robust training directly on the \q model but hoping it will react to the adversarial examples in the same manner as its \fp version. Thus we introduce the combination of \name-based adversarial training and knowledge distillation during quantization aware training. We hope the process of distillation will reduce the deviation between the full-presicion model and the \q model.

\paragraph{Defensive quantization.}

This method regularizes the Lipschitz constants of the \q model to defend against the PGD attack~\cite{defensive_q}. It is in principle subsumed by Minimax PGD robust training because it makes the quantized model differ \emph{more} from the \fp model than without any defense. We were unable to obtain the code from the authors, so we omit it from our evaluation.
